An Integrated Programmable CPG with Bounded Output

Cyclic motions are fundamental patterns in robotic applications including industrial manipulation and legged robot locomotion. This paper proposes an approach for the online modulation of cyclic motions in robotic applications. For this purpose, we present an integrated programmable Central Pattern Generator (CPG) for the online generation of the reference joint trajectory of a robotic system out of a library of desired periodic motions. The reference trajectory is then followed by the lower-level controller of the robot. The proposed CPG generates a smooth reference joint trajectory convergence to the desired one while preserving the position and velocity joint limits of the robot. The integrated programmable CPG consists of one novel bounded output programmable oscillator. We design the programmable oscillator for encoding the desired multidimensional periodic trajectory as a stable limit cycle. We also use the state transformation method to ensure that the oscillator's output and its first-time derivative preserve the joint position and velocity limits of the robot. With the help of Lyapunov-based arguments, We prove that the proposed CPG provides the global stability and convergence of the desired trajectory. The effectiveness of the proposed integrated CPG for trajectory generation is shown in a passive rehabilitation scenario on the Kuka iiwa robot arm, and also in a walking simulation on a seven-link bipedal robot.

==> sections/Abstract0.tex <==
% As a general rule, do not put math, special symbols or citations
% in the abstract or keywords.
\begin{abstract}
	Cyclic motions are fundamental patterns in robotic applications including industrial manipulation and legged robot locomotion.
	This paper proposes an approach for online modulation of cyclic motion in robotic applications.
	For this purpose, we present an integrated Central Pattern Generator (CPG) for online generation of reference joint trajectory of the robotic system from a library of desired periodic ones resulting in the desired cyclic motions.
	The reference trajectory is followed by the joint control system of the robot.
	The proposed integrated CPG generates a smooth reference joint trajectory converging to the desired one while preserving the position and velocity joint limits of the robot.
	The integrated CPG consists of one novel bounded output programmable oscillator.
	We design the programmable oscillator for encoding the desired multidimensional periodic trajectory as a stable limit cycle.
	We also use the state transformation method to ensure that the oscillator's output and its first time derivative preserve the joint position and velocity limits of the robot.
	We prove that the proposed integrated CPG provides the global stability and convergence of the desired trajectory with the help of Lyapunov based arguments.
	The soundness of the proposed integrated CPG for trajectory generation is validated in passive rehabilitation experiment on the Kuka iiwa arm, and also in walking simulation on a seven-link bipedal robot.
\end{abstract}

% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
	smooth motion modulation, cyclic motions, integrated central pattern generator (CPG), state constrained dynamical system, programmable oscillator.
\end{IEEEkeywords}


==> sections/Appendices0.tex <==
% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%

\appendices
\section{Proof of Theorem \ref{thm:stabilityOfProgrammableOscillator}}
\label{app:MDVOstability}

Theorem \ref{thm:stabilityOfProgrammableOscillator} has 3 items that we prove them in the following.

\begin{figure}[!t]
	\centering
	\subfloat{
		\includegraphics[width=0.45\linewidth]{Figures/compareTrackingError.eps}
		\includegraphics[width=0.45\linewidth]{Figures/compareTorqueSummation.eps}
	}
	\caption{The convergence rate and control effort of the seven-link biped using the integrated CPG in AS and AOS modes and during the transition motion from standing to walking with step length of $50 (cm)$ and step period of $2 (sec)$.
		The left and right figures depict $\left\|\be_1\right\| = \left\| \bs_1-\bg_p\right\|$ and the integral of $\left\|\tau\right\|$ where $\tau$ is the vector of joint actuator torques of the robot.}
	\label{fig:sevenLinkBiped_compareASandAOS}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{$\bx(t)$ is bounded and converges to $\bq_d (\varphi)$ from any $\bx(0)$}

Starting with
\begin{equation}
\label{eq:Lyapunov_1}
V_1 \left( \bx , \varphi \right) = \dfrac{1}{2} \be_{\bs}^\top B \be_{\bs} + \dfrac{1}{2} \be_{\dbs}^\top \be_{\dbs},
\end{equation} 
where $\left[ \be_{\bs}^\top,\be_{\dbs}^\top \right] = \bx^\top - \bq_d^\top(\varphi) = \left[\bs^\top-\bbf^\top (\varphi) ,\dbs^\top - \bbf^{\prime \top} (\varphi) \right]$, we compute the time derivative of $V_1$ along the trajectories of the system \eqref{eq:MDVO_dynamic} to obtain
\begin{equation}
\dot{V}_1 = -\gamma \left( \be_{\bs}^\top B \pbf + \be_{\dbs}^\top \ppbf \right)^2 - \be_{\dbs}^\top A \be_{\dbs}.
\end{equation}
Sine $A$ is a positive definite matrix and $\gamma$ is a nonnegative constant, $\dot{V}_1 \leq 0$.
Moreover, \eqref{eq:Lyapunov_1} shows that $V_1 \geq 0$ where $V_1 = 0$ iff $\left[\be_{\bs},\be_{\dbs}\right] = \left[\mathbf{0}_n,\mathbf{0}_n\right]$.
Hence $\be_{\bs}$ and $\be_{\dbs}$ are bounded.
Assuming that $\bbf(t)$ and its first time derivative are bounded, one also concludes the boundedness of $\bx(t)$ for any initial condition.
In order to get convergence of $\bq_d(\varphi)$ (or $\left[\be_{\bs},\be_{\dbs}\right] = \left[\mathbf{0}_n,\mathbf{0}_n\right]$), it is sufficient to examine the largest invariant subset of the set $\Omega = \left\{\left[\bx^\top,\varphi\right] : \dot{V}_1 = 0 \right\}$.
Considering \eqref{eq:MDVO_dynamic}, it is possible to verify that $\left\{ \left[\bq_d^\top (\varphi),\varphi \right] \right\}$ is the only invariant subset of $\Omega$.
Therefore, we can conclude the convergence of $\bx = \bq_d(\varphi)$ according to the LaSalle Lemma \cite{khalil2002nonlinear}.
The global convergence of $\bx = \bq_d(\varphi)$ is the consequence of the radially unbounded property of $V_1$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{if $\gamma = 0$, then $\left[\bq_d^\top (t + \varphi (0)), t + \varphi (0)\right]^\top$ is globally AS}

If $\gamma = 0$, then we have $\dot{\varphi} = 1$, and thus $\varphi = t + \varphi(0)$.
Hence, the system \eqref{eq:MDVO_dynamic} is simplified to the $2n$ dimensional system whose state space vector is $\bx$.
Accordingly, the function $V_1$ is the Lyapunov function of the system, and thus the global AS of $\bq_d(t+\varphi(0)) = {\small\left[\bbf^\top (t+\varphi(0)),\bbf^{\prime \top} (t+\varphi(0))\right]^\top}$ is concluded based on the Lyapunov stability theorem \cite{khalil2002nonlinear}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{if $\gamma \rightarrow \infty$, then $\bx = \bq_d (t)$ is the globally stable limit cycle}

To investigate the stability of the set $\bq_d(t)$, we prove that for $\gamma \rightarrow \infty$,
\begin{itemize}
	\item $\forall \left[\bx^\top,\varphi\right] \in \mathcal{P}_{\bbf}, V_1(\bx, \varphi) = 0$,
	 \item $\forall \left[\bx^\top,\varphi\right] \notin \mathcal{P}_{\bbf}, V_1(\bx, \varphi) > 0$, and
	 \item $\forall \left[\bx^\top,\varphi\right] \notin \mathcal{P}_{\bbf}, \dot{V}_1(\bx, \varphi) < 0$.
\end{itemize}
Thus, one can conclude that $\mathcal{P}_{\bbf}$ is the stable limit cycle of the system \eqref{eq:MDVO_dynamic} according to the extension of the Lyapunov stability theorem for invariant sets \cite{zubov1964methods}.
The global stability of the limit cycle $\mathcal{P}_{\bbf}$ is the result of the radially unbounded property of $V_1$.
For this purpose, we prove that for $\gamma \rightarrow \infty$, $\left[\be_{\bs},\be_{\dbs}\right] = \left[\mathbf{0}_n,\mathbf{0}_n\right]$ iff $\left[\bx^\top,\varphi\right] \in \mathcal{P}_{\bbf}$.
Since $\be_{\bs} = \bs - \bbf(\varphi)$ and $\be_{\dbs} = \dbs - \pbf(\varphi)$, one can figure out that if $\be_{\bs}=\be_{\dbs} = \mathbf{0}_n$, then $\left[\bx^\top,\varphi\right] \in \mathcal{P}_{\bbf}$.
To prove that for $\left[\bx^\top,\varphi\right] \in \mathcal{P}_{\bbf}$, we have $\be_{\bs}=\be_{\dbs} = \mathbf{0}_n$, we show that for $\gamma \rightarrow \infty$ and $\left[\bx^\top,\varphi\right] \in \mathcal{N}_\delta$ where $\mathcal{N}_\delta$ is the $\delta$-neighborhood of $\mathcal{P}_{\bbf}$, $\bq_d(\varphi)$ is the point from the curve of $\mathcal{P}_{\bbf}$ in the shape space having the minimum distance from the current shape states.
In this regard, we define the distance between $\bx = {\small \left[\bs^\top,\dbs^\top\right]^\top}$ and the curve of $\mathcal{P}_{\bbf}$ in the shape space as
\begin{equation}
\dist \left( \bx,\mathcal{P}_{\bbf} \right) = \min_{\tau \in [0,T]} \dis(\bx,\bq_d(\tau)).
\end{equation}
where $T \in \mathbb{R}^+$ is the period of $\bq_d(t)$, and
\begin{equation}
\label{eq:EDVO_ptpDistance}
\begin{aligned}
\dis (\bx,\bq_d(\tau)) = &\dfrac{1}{2}\left(\bs - \bbf(\tau)\right)^\top B \left(\bs - \bbf(\tau) \right)\\
& + \dfrac{1}{2}\left(\dbs - \pbf(\tau) \right)^\top \left(\dbs - \pbf(\tau) \right).
\end{aligned}
\end{equation}

In the following, we prove that $\dis(\bx,\bq_d(\varphi)) = \dist(\bx,\mathcal{P}_{\bbf})$ if $\gamma \rightarrow \infty$.
Since $\dis(\bx,\bq_d(\varphi))$ is continuous, its extreme is at $\dfrac{\partial \dis  (\bx,\bq_d(\varphi))}{\partial \varphi} = 0$.
Thus, we consider the first and second derivatives of $\dis (\bx, \bq_d(\varphi))$ w.r.t. the phase state, \ie
{\small
	\begin{equation}
	\label{eq:EDVO_dpp}
	\begin{aligned}
	&\dis_\varphi = \dfrac{\partial \dis  (\bx,\bq_d(\varphi))}{\partial \varphi} = - \left(\bs-\bbf\right)^\top B \pbf - \left( \dbs - \pbf \right)^\top \ppbf, \\
	&\dis_{\varphi \varphi} = \dfrac{\partial^2 \dis (\bx,\bq_d(\varphi))}{\partial \varphi^2} = \bbf^{\prime \top} B \bbf^\prime + \bbf^{\prime \prime \top} \bbf^{\prime \prime}\\
	& \qquad \qquad \qquad \qquad \qquad - \left(\bs-\bbf\right)^\top B \ppbf - \left(\dbs - \pbf\right)^\top \pppbf.
	\end{aligned}
	\end{equation}
}
The lower bound of $\dis_{\varphi \varphi}$ is as
{\small
	\begin{equation}
	\label{eq:EDVO_dppLowerBound}
	\begin{aligned}
	\dis_{\varphi\varphi} \geq{} &\bbf^{\prime \top} B \bbf^\prime + \bbf^{\prime \prime \top} \bbf^{\prime \prime} \\
	&- \left\|\beta^{1/2} (\bs-\bbf)\right\| \left\|B^{1/2}\ppbf\right\| - \left\|\dbs - \pbf\right\| \left\|\pppbf\right\|.
	\end{aligned}
	\end{equation}
}
On the other hand, considering \eqref{eq:EDVO_ptpDistance}, we have
\begin{equation}
\begin{aligned}
&\left\|B^{1/2} (\bs-\bbf)\right\| \leq \sqrt{2 \dis (\bx,\bq_d(\varphi))}, \\
&\left\|\dbs-\pbf\right\| \leq \sqrt{2 \dis (\bx,\bq_d(\varphi))}.
\end{aligned}
\end{equation}
Considering the above relations, \eqref{eq:EDVO_dppLowerBound} is simplified as
\begin{equation}
\label{eq:EDVO_dppLowerBound_simple}
{\footnotesize
\dis_{\varphi\varphi} \geq \bbf^{\prime \top} B \pbf + \bbf^{\prime \prime \top} \ppbf - \left( \ppbf_m + \pppbf_m \right) \sqrt{2 \dis (\bx,\bq_d(\varphi))}},
\end{equation}
where $\ppbf_m = \max_\varphi \left(\left\| B^{1/2} \ppbf\right\|\right)$ and $\pppbf_m = \max_\varphi \left(\left\| \pppbf\right\|\right)$.
Since $B$ is positive definite and $\not\exists \varphi$ that $\pbf(\varphi) = \ppbf(\varphi) = \mathbf{0}_n$, one can find $\delta \in \mathbb{R}^+$ such that $\forall \left[\bx^\top,\varphi\right] \in \mathcal{N}_\delta$ where $\mathcal{N}_\delta$ is the $\delta$-neighborhood of $\mathcal{P}_{\bbf}$, we have $\dis_{\varphi\varphi} > 0$.
As a result, $\forall \left[\bx^\top,\varphi\right] \in \mathcal{N}_\delta$, $\dis(\bx,\bq_d(\varphi)) = \dist(\bx,\mathcal{P}_{\bbf})$ iff $\dis_{\varphi \varphi} = 0$.
To investigate time evolution of $\dis_\varphi$, we compute its time derivative along the trajectories of \eqref{eq:MDVO_dynamic} as
{\small\begin{equation}
	\label{eq:EDVO_dphiDyn}
	\begin{aligned}
	\dot{\dis} _\varphi = & - \left( \bbf^{\prime \top} B \pbf + \bbf^{\prime \prime \top} \ppbf - e_{\bs}^\top B \ppbf - e_{\dbs}^\top \pppbf \right) \gamma \dis _\varphi\\
	&- \left( \bbf ^{\prime \top} B - \bbf^{\prime \prime \top} A + \bbf^{\prime \prime \prime \top} \right) e_{\dbs}.
	\end{aligned}
	\end{equation}}
Considering $V_2 = \frac{1}{2} \dis_{\varphi}^2$, the time derivative of $V_2$ is as
\begin{equation}
{\footnotesize
\begin{aligned}
\dot{V}_2 \leq - &\left( \bbf^{\prime \top} B \pbf + \bbf^{\prime \prime \top} \ppbf - \left( \ppbf_m + \pppbf_m \right) \sqrt{2 \dis(\bx,\bq_d(\varphi))} \right)\\
& \, \gamma \dis _\varphi^2 + \eta |\dis_\varphi| \sqrt{2 \dis (\bx,\bq_d(\varphi))}.
\end{aligned}}
\end{equation}
where $\eta = \max_\varphi \left(\left|\bbf^{\prime \top} B - \bbf^{\prime \prime \top} A + \bbf^{\prime \prime \prime \top}\right|\right)$.
Since $\dis (\bx,\bq_d(\varphi)) = V_1$, and $\dot{V}_1 \leq 0$, we have $\max_{\left[\bx^\top,\varphi\right] \in \mathcal{N}_\delta} \dis (\bx,\bq_d(\varphi)) = d_0 = \dis (\bx(t_\delta),\bq_d(\varphi(t_\delta)))$.
Thus, we have
\begin{equation}
	\begin{aligned}
	\dot{V}_2 \leq - &\left( \bbf^{\prime \top} B \pbf + \bbf^{\prime \prime \top} \ppbf - \left( \ppbf_m + \pppbf_m \right) \sqrt{2 d_0} \right)\\
	& \, \gamma \dis _\varphi^2 + \eta |\dis_\varphi| \sqrt{2 d_0}.
	\end{aligned}
\end{equation}
Hence, for every $\epsilon \in (0,1)$ if
\begin{equation}
\label{eq:EDVO_eq2}
| \dis _\varphi | \geq \dfrac { \alpha \sqrt{2 d_0} }{\epsilon \gamma \left(\bbf^{\prime \top} B \pbf + \bbf^{\prime \prime \top} \ppbf - \left( \ppbf_m + \pppbf_m \right) \sqrt{2 d_0} \right) },
\end{equation}
we have
\begin{equation}
\begin{aligned}
	\dot{V}_2 & \leq - (1-\epsilon) \left( \bbf^{\prime \top} B \pbf + \bbf^{\prime \prime \top} \ppbf - \left( \ppbf_m + \pppbf_m \right) \sqrt{2 d_0} \right) \gamma \dis _\varphi^2\\
	& \leq - (1-\epsilon) \gamma \dis _\varphi^2.
\end{aligned}
\end{equation}
Therefore, $\dis_{\varphi}^2$ decreases when the trajectory enters $\mathcal{N}_\delta$.
On the other hand, we have
\begin{equation}
- \dis_{\varphi}^2 (t_\delta) = 2 \int_{t_\delta}^{t_\nu} \dot{V}_2 dt \leq - (1-\epsilon) \gamma \int_{t_\delta}^{t_\nu} \dis _\varphi^2 dt,
\end{equation}
where $t_\delta \in \mathbb{R}^+$ is the time instance that the trajectory of the system enters $\mathcal{N}_\delta$, and $t_\nu > t_\delta$ is the time instance when $\dis_{\varphi}^2 (t_\nu) = 0$.
From the above equation, one can concludes that $\lim\limits_{\gamma \rightarrow \infty} t_\nu = t_\delta$.
Hence, if $\gamma \rightarrow \infty$, for all $\left[\bx^\top,\varphi\right] \in \mathcal{N}_\delta$, we have $\dis_\varphi = 0$, and thus $\lim\limits_{\gamma \rightarrow \infty} \dis (\bx,\bq_d(\varphi)) = \dist (\bx,\mathcal{P}_{\bbf})$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of Theorem \ref{thm:psiDefinable}}
\label{app:psiDefinable}

Substituting \eqref{eq:BMDVO_stateTransformation}
into \eqref{eq:BMDVO_constrainedForPsi}, we have
\begin{equation}
\begin{aligned}
\breve{\delta}_{\by}^2 \breve{\delta}_{\dot{\by}} \left| \tanh{(\bg_v)} \right| \leq &\left|
\breve{\delta}_{\by}^2 - \breve{\delta}_{\by}^2 \tanh^2 {(\breve{\bg}_p)}\right| \delta_{\dot{\by}} \\
& = \breve{\delta}_{\by}^2 \left| I_n - \tanh^2 {(\breve{\bg}_p)} \right| \delta_{\dot{\by}}.
\end{aligned}
\end{equation}
The above inequality is simplified as
\begin{equation}
\breve{\delta}_{\by} \left| J_{\bg_p}^{-1} \tanh{(\bg_v)} \right| \leq \mathbf{1}_n.
\end{equation}
According to the above inequality and the fact that ${\left| \breve{\delta}_{\by}^{-1} J_{\bs_1} \right| \leq \mathbf{1}_n}$, one concludes that
\begin{equation}
\left| J_{\bs_1} J_{\bg_p}^{-1} \tanh{(\bg_v)} \right| \leq \mathbf{1}_n.
\end{equation}
Thus, the variable $\bsi$ is definable.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{Proof of Theorem \ref{thm:BMDVO}}
\label{app:BMDVO}

Theorem \ref{thm:BMDVO} has 4 items that we prove them in the following.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{$\bx(t)$ is bounded and converges to $\bx^*(\varphi)$ from any initial condition}

As the trajectory $\left[ \bs_1^\top,\bs_2^\top,\varphi\right] = \left[ \bg_p^\top,\bg_v^\top,\varphi\right]$ satisfies the differential equations \eqref{eq:BMDVO_Dynamics}, ${\small\left[\bx^{* ^\top},\varphi\right]^\top} = \left[ \bg_p^\top,\bg_v^\top,\varphi \right]^\top$ is the response of the bounded output programmable oscillator for the initial condition $\left[ \bg_p^\top\left(\varphi(0)\right),\bg_v^\top\left(\varphi(0)\right),\varphi(0) \right]^\top$.
To prove the bounded property of $\bx^*$, we consider
\begin{equation}
	V_3 = \dfrac{1}{2}
\begin{bmatrix}
\be_1^\top & \be_2^\top
\end{bmatrix}
P
\begin{bmatrix}
\be_1 \\ \be_2
\end{bmatrix}
\end{equation}
where $\be_1 = \bs_1 - \bg_p$, $\be_2 = \bs_2 - \bsi$ and
\begin{equation}
\label{eq:app_pMatrix}
P = \begin{bmatrix}
C & A \\
A & B
\end{bmatrix}.
\end{equation}
As $A$, $B$, $C$ and $BA^{-1}C-A$ are diagonal positive definite matrices, $V_3$ is a PSD based on the Schur complement for block matrices \cite{zhang2006schur}.
Note that $V_3 = 0$ iff $\left[\be_1^\top,\be_2^\top\right] = \left[\mathbf{0}_n^\top,\mathbf{0}_n^\top\right]$.

The time derivative of $V_3$ along the trajectories of the bounded output programmable oscillator is as
\begin{equation}
{\small
\begin{aligned}
	\dot{V}_3 ={} &\be_2^\top \left(A-BA^{-1}C\right)J_{\bs_1}^{-1}\breve{\delta}_{\dot{\by}} \big( \tanh{(\bs_2)}-\tanh{(\bsi)} \big)\\
& - \left\| A \be_1 + B \be_2 \right\|^2 -\gamma W^2,
\end{aligned}}
\end{equation}
where
\begin{equation}
\begin{aligned}
W = \left( \be_1^\top C + \be_2^\top A \right) J_{\bg_p}^{-1} \breve{\delta}_{\dot{\by}} \tanh{(\bg_v)}\\
 + \left( \be_1^\top A + \be_2^\top B \right) \bsi_\varphi.
\end{aligned}
\end{equation}
As $BA^{-1}C-A$, $J_{\bs_1}$ and $\breve{\delta}_{\dot{\by}}$ are diagonal PD matrices, and $\gamma$ is a non-negative constant, $\dot{V}_3 \leq 0$.
Thus, $\be_1$ and $\be_2$ are bounded.
Moreover, as $V_3$ is radially unbounded w.r.t. $\left\| \left[\be_1^\top,\be_2^\top \right]\right\|$, one can conclude that $\be_1$ and $\be_2$ are bounded from any initial condition.
In conclusion, if $\bbf(t) \in \mathcal{Q}$, then the shape state vector $\bx$ is bounded for any initial condition.

In order to get the convergence of $\bx^*$, it is sufficient to examine the largest invariant subset of $\Gamma = \left\{\left[\bx^\top, \varphi\right]\right\}: \dot{V}_3 = 0$.
Considering the dynamic \eqref{eq:BMDVO_Dynamics}, it is possible to verify that $\left\{\left[\bx^{*^\top}, \varphi\right]\right\}$ is the only invariant subset of $\Gamma$.
Therefore, we can conclude the convergence of $\bx^*$ according to the LaSalle Lemma \cite{khalil2002nonlinear}.
The global convergence of $\bx^*$ is the consequent of the radially unbounded property of $\dot{V}_3$ w.r.t. $\left\|\bx-\bx^*\right\|$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{if $\gamma = 0$, $\left[\bx^{* \top}(t+\varphi(0)),t+\varphi(0)\right]^\top$ is globally AS}

For $\gamma = 0$, \eqref{eq:BMDVO_phaseDynamic} is simplified to $\dot{ \varphi } = 1$, and thus $\varphi(t) = t + \varphi(0)$.
Hence, the system \eqref{eq:BMDVO_Dynamics} is simplified to the $2n$ dimensional system whose state space vector is $\bx$.
Accordingly, the function $V_3$ is the Lyapunov function of the system, and thus the global AS of ${\small\left[\bg_p^\top (t+\varphi(0)),\bg_v^\top (t+\varphi(0))\right]^\top}$ is concluded based on the Lyapunov stability theorem \cite{khalil2002nonlinear}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{if $\gamma \rightarrow \infty$, $\bx^*(t)$ is the globally stable limit cycle}

$\bx^*(t)$ is the globally stable limit cycle iff $\mathcal{P}_{\bg}$ is globally AS where $\mathcal{P}_{\bg}$ is the set of the states belonging to $\bx^*(t)$, \ie \cite{khalil2002nonlinear}
\begin{equation}
\mathcal{P}_{\bg} = \left\{ \left[ \bs_1^\top, \bs_2^\top, \varphi \right] \, : \, \exists \varphi, \, \bs_1=\bg_p(\varphi),\bs_2=\bg_v(\varphi) \right\}.
\end{equation}
To investigate the AS of the set $\mathcal{P}_{\bg}$, we prove that for $\gamma \rightarrow \infty$,
\begin{itemize}
	\item $\forall \left[\bx^\top,\varphi\right] \in \mathcal{P}_{\bg}, V_3(\bx, \varphi) = 0$,
	\item $\forall \left[\bx^\top,\varphi\right] \notin \mathcal{P}_{\bg}, V_3(\bx, \varphi) > 0$, and
	\item $\forall \left[\bx^\top,\varphi\right] \notin \mathcal{P}_{\bg}, \dot{V}_3(\bx, \varphi) < 0$.
\end{itemize}
Thus, one can conclude that $\mathcal{P}_{\bg}$ is the stable limit cycle of the system \eqref{eq:BMDVO_Dynamics} according to the extension of the Lyapunov stability theorem for invariant sets \cite{zubov1964methods}.
The global stability of the limit cycle $\mathcal{P}_{\bg}$ is the result of the radially unbounded property of $V_3$.
For this purpose, we prove that for $\gamma \rightarrow \infty$, $\left[\be_1,\be_2\right] = \left[\mathbf{0}_n,\mathbf{0}_n\right]$ iff $\left[\bx^\top,\varphi\right] \in \mathcal{P}_{\bg}$.
Since $\be_1 = \bs_1 - \bg_p(\varphi)$ and $\be_2 = \bs_2 - \bg_v(\varphi)$, one can figure out that if $\be_1=\be_2 = \mathbf{0}_n$, then $\left[\bx^\top,\varphi\right] \in \mathcal{P}_{\bg}$.
To prove that for $\left[\bx^\top,\varphi\right] \in \mathcal{P}_{\bg}$, we have $\be_1=\be_2 = \mathbf{0}_n$, we show that for $\gamma \rightarrow \infty$ and $\left[\bx^\top,\varphi\right] \in \mathcal{N}_\rho$ where $\mathcal{N}_\rho$ is the $\rho$-neighborhood of $\mathcal{P}_{\bg}$, $\bx^*(\varphi)$ is the point from the curve of $\mathcal{P}_{\bg}$ in the shape space having the minimum distance from the current shape states.
In this regard, we define the distance between $\bx = {\small \left[\bs_1^\top,\bs_2^\top\right]^\top}$ and the curve of $\mathcal{P}_{\bg}$ in the shape space as
\begin{equation}
\dist(\bx,\mathcal{P}_{\bg}) = \min_{\tau \in \left[0,T\right]} \dis(\bx,\bx^*(\tau)),
\end{equation}
where $T \in \mathbb{R}^+$ is the period of $\bbf(t)$ and $\dis(\bx,\bx^*(\tau))$ is as
\begin{equation}
\label{eq:app_BMDVO_distancDef}
\begin{aligned}
	\dis(\bx,\bx^*(\tau)) ={}& \dfrac{1}{2}
	\left[
	\left(\bs_1-\bg_p(\tau)\right)^\top, \left(\bs_2-\bg_v(\tau)\right)^\top
	\right]\\
	&P
	\begin{bmatrix}
	\bs_1-\bg_p(\tau) \\ \bs_2-\bs_v(\tau)
	\end{bmatrix}.
\end{aligned}
\end{equation}
In the following, we prove that $\dis(\bx,\bx^*(\varphi)) = \dist(\bx,\mathcal{P}_{\bg})$ if $\gamma \rightarrow \infty$.
Since $\dis(\bx,\bx^*(\varphi))$ is continuous, its extreme is at $\dfrac{\partial \dis  (\bx,\bx^*(\varphi))}{\partial \varphi} = 0$.
Thus, we consider the first and second derivatives of $\dis (\bx, \bx^*(\varphi))$ w.r.t. the phase state, \ie
\begin{equation}
\begin{aligned}
& \dis_\varphi = \dfrac{\partial \dis}{\partial \varphi} (\bx,\bx^*) =
- \begin{bmatrix}
\be_1^\top & \be_2^\top
\end{bmatrix}
P
\begin{bmatrix}
\bg^\prime_p \\ \bsi_\varphi
\end{bmatrix}, \\
&\dis_{\varphi \varphi} = \dfrac{\partial^2 \dis}{\partial \varphi^2} (\bx,\bx^*) = 
- \begin{bmatrix}
\be_1^\top & \be_2^\top
\end{bmatrix}
P
\begin{bmatrix}
\bg^{\prime \prime}_p \\ \bsi^{\prime \prime}
\end{bmatrix}\\
& \qquad \qquad \qquad \qquad \quad + \begin{bmatrix}
\bg_p^{\prime \top} & \bsi^\top_\varphi
\end{bmatrix}
P
\begin{bmatrix}
\bg^\prime_p \\ \bsi_\varphi
\end{bmatrix}.
\end{aligned}
\end{equation}
The lower bound of $\dis_{\varphi \varphi}$ is as
\begin{equation}
\label{eq:app_lowerBoundDff}
\dis_{\varphi\varphi} \geq \underline{\lambda} \begin{Vmatrix}
\bg_p^{\prime \top} & \bsi^\top_\varphi
\end{Vmatrix}^2
- \kappa \sqrt{2 \dis (\bx,\bx^*)},
\end{equation}
where $\underline{\lambda}$ is the minimum eigenvalue of $P$, and $\kappa = \max_\varphi \left\| P^{1/2} 
\begin{bmatrix}
\bg_p^{\prime \prime} & \bsi_{\varphi \varphi}
\end{bmatrix} \right\|$.
Note that $C-AB^{-1}A $ is PD, thus $\underline{\lambda} > 0$.
Since $\underline{\lambda}$ is positive and $\not\exists \varphi$ that $\bg_p^\prime(\varphi) = \bsi_\varphi(\varphi) = \mathbf{0}_n$, one can find $\rho \in \mathbb{R}^+$ such that $\forall \left[\bx^\top,\varphi\right] \in \mathcal{N}_\rho$ where $\mathcal{N}_\rho$ is the $\rho$-neighborhood of $\mathcal{P}_{\bg}$, we have $\dis_{\varphi\varphi} > 0$.
As a result, $\forall \left[\bx^\top,\varphi\right] \in \mathcal{N}_\rho$, $\dis(\bx,\bx^*(\varphi)) = \dist(\bx,\mathcal{P}_{\bg})$ iff $\dis_{\varphi \varphi} = 0$.
To investigate time evolution of $\dis_\varphi$, we compute its time derivative along the trajectories of \eqref{eq:BMDVO_Dynamics} as
\begin{equation}
{\small
	\label{eq:app_BMDVO_dppDiff}
	\begin{aligned}
	\dot{\dis} _\varphi = &- \left( \begin{bmatrix}
	\bg_p^{\prime \top} & \bsi^{\top}_\varphi
	\end{bmatrix} P \begin{bmatrix}
	\bg_p^{\prime \top} \\ \bsi^{\top}_\varphi
	\end{bmatrix} 
	- \begin{bmatrix}
	\be_1^\top & \be_2^\top
	\end{bmatrix} P \begin{bmatrix}
	\bg_p^{\prime \prime} \\ \bsi_{\varphi \varphi}
	\end{bmatrix} \right) \gamma \dis _\varphi \\
	&- \begin{bmatrix}
	\be_1^\top & \be_2^\top
	\end{bmatrix} \left( P
	\begin{bmatrix}
	\bg_p^{\prime \prime} \\ \bsi_{\varphi \varphi} + \dot{\bsi}_\varphi
	\end{bmatrix}
	- \begin{bmatrix}
	A^2 & AB \\ BA & B^2
	\end{bmatrix} \begin{bmatrix}
	\bg^\prime_p \\ \bsi_\varphi
	\end{bmatrix}\right) \\
	&- \left( \tanh{(\bs_2)} - \tanh{(\bsi)} \right) J_{\bs_1}^{-1} \breve{\delta}_{\dot{\by}} \left( A-A^{-1}CB \right) \bsi_\varphi
	\end{aligned}}
\end{equation}
Considering $V_4 = \frac{1}{2} \dis_{\varphi}^2$, the time derivative of $V_4$ is as
\begin{equation}
\label{eq:app_BMDVO_V11Diff}
\begin{aligned}
\dot{V}_4 = \dis_\varphi \dot{\dis}_\varphi \leq {}& - \left( \underline{\lambda} 
\begin{Vmatrix}
\bg_p^{\prime \top} & \bsi^{\top}_\varphi
\end{Vmatrix}^2
- \kappa \sqrt{2 d_0} \right) \gamma \dis _\varphi^2 \\
&+ \rho(d_0) |\dis_\varphi|,
\end{aligned}
\end{equation}
where
\begin{equation}
\rho(d) = \sqrt{2 d_0} \left( \kappa + \upsilon \right)
+ 2  \tanh(\sqrt{2 d_0}\mu)
\end{equation}
and $\upsilon = \max_\varphi \left( \left\| \begin{bmatrix}
A^2 & AB \\ BA & B^2
\end{bmatrix} \begin{bmatrix}
\bg^\prime_p \\ \bsi_\varphi
\end{bmatrix} \right\| \right)$
and ${\mu = \max_\varphi \left( J_{\bs_1}^{-1} \breve{\delta}_{\dot{\by}} \left( A-A^{-1}CB \right) \bsi_\varphi \right)}$.
Based on \eqref{eq:app_BMDVO_V11Diff}, for $\epsilon \in (0,1)$ if 
\begin{equation}
\label{eq:app_BMDVO_AOSregion}
| \dis _\varphi | \geq \dfrac { \rho(d_0) }{\epsilon \gamma \left( \underline{\lambda} \begin{Vmatrix}
	\bg_p^{\prime \top} & \bsi^{\top}_\varphi
	\end{Vmatrix}^2
	- \kappa \sqrt{2 d_0} \right) },
\end{equation}
then we have
\begin{equation}
\dot{V}_4 \leq - (1-\epsilon) \left( \underline{\lambda} \begin{Vmatrix}
\bg_p^{\prime \top} & \bsi^{\top}_\varphi
\end{Vmatrix}^2
- \kappa \sqrt{2 d_0} \right) \gamma \dis _\varphi^2.
\end{equation}
Therefore, $\dis_{\varphi}^2$ decreases when the trajectory enters $\mathcal{N}_\rho$.
On the other hand, we have
\begin{equation}
- \dis_{\varphi}^2 (t_\rho) = 2 \int_{t_\rho}^{t_\nu} \dot{V}_4 dt \leq - (1-\epsilon) \gamma \xi \int_{t_\delta}^{t_\nu} \dis _\varphi^2 dt,
\end{equation}
where $t_\rho \in \mathbb{R}^+$ is the time instance that the trajectory of the system enters $\mathcal{N}_\rho$, $t_\nu > t_\rho$ is the time instance when $\dis_{\varphi}^2 (t_\nu) = 0$, and $\xi = \min \left| \underline{\lambda} \begin{Vmatrix}
\bg_p^{\prime \top} & \bsi^{\top}_\varphi
\end{Vmatrix}^2
- \kappa \sqrt{2 d_0} \right|$.
From the above equation, one can concludes that $\lim\limits_{\gamma \rightarrow \infty} t_\nu = t_\rho$.
Hence, if $\gamma \rightarrow \infty$, for all $\left[\bx^\top,\varphi\right] \in \mathcal{N}_\rho$, we have $\dis_\varphi = 0$, and thus $\lim\limits_{\gamma \rightarrow \infty} \dis (\bx,\bx^*(\varphi)) = \dist (\bx,\mathcal{P}_{\bg})$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{the output $\by(t)$ converges to the curve of $\bq_d(t)$ in the space $\left(\by,\dot{ \by }\right)$ while $\by(t) \in \mathcal{Q}$}

As $\bx$ converges to $\bx^*(\varphi)$, $\by(t)$ converges to the curve of $\bq_d(t)$ in the shape $(\by,\dot{ \by })$.
Moreover, according to the definition of $\by$ in \eqref{eq:BMDVO_Dynamics} and the fact that $\bx$ is bounded, we have ${\by_{min}=\by_{avg} - \delta_{\by} < \by < \by_{avg} + \delta_{\by} = \by_{max}}$.
In addition, based on the dynamic of the bounded output programmable oscillator, the time derivative of the output is as
\begin{equation}
\dot{\by} = \delta_{\dot{y}} \tanh{(\bs_1)}. 
\end{equation}
Thus, one concludes that $ |\dot{\by}| \leq \delta_{\dot{y}}$.
In conclusion, we have $\by(t) \in \mathcal{Q}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> sections/BoundedOutputProgrammableOscillator0.tex <==
\section{Bounded Output Programmable Oscillator}
\label{sec:boundedOutputProgrammableOscillator}

Using the programmable oscillator, we can generate a smooth trajectory tracking the desired periodic one, and use it as the reference joint trajectory for a robot controller for generating the desired cyclic motion from any initial condition.
The reference trajectory is feasible for the robot if it preserves its physical limits including position and velocity joint limits.
In this section, we modify the dynamic of the programmable oscillator for generating a bounded output preserving the predefined limits for the output and its first time derivative.

Assume that the feasible region for the output of the programmable oscillator is as
\begin{equation}
\label{eq:EDVO_outputConstrained}
\mathcal{Q} := \left\{ \by \in \mathbb{R}^n \, : \, \by_{min} < \by < \by_{max}, \ |\dot{\by}| < \delta_{\dot{\by}} \right\}.
\end{equation}
$\by_{min}, \by_{max} \in \mathbb{R}^n$ are vectors of the minimum and maximum feasible value of the output, respectively, and ${\delta_{\dot{\by}} \in \mathbb{R}^n}$ is the vector of the maximum feasible rate of change of the output.

For generating a feasible output, we define the output of the bounded output programmable oscillator as \cite{charbonneau2016line}
\begin{equation}
\label{eq:EDVO_outputDefinition}
\by = \by_{avg} + \breve{\delta}_{\by} \tanh{(\bs_1)},
\end{equation}
where $\by_{avg} = \frac{\by_{max}+\by_{min}}{2}$, $\breve{\cdot} = \diag(\cdot)$, and ${\delta_{\by} = \frac{\by_{max}-\by_{min}}{2}}$.
$\bx = \left[\bs_1^\top, \bs_2^\top\right]^\top \in \mathbb{R}^{2n}$ is the shape state vector of the bounded output programmable oscillator.
If $\bs_1$ is bounded, the above equation guarantees that ${\by_{min} = \by_{avg} - \delta_{\by} < \by < \by_{avg} + \delta_{\by} = \by_{max}}$.

For preserving the limitation of the rate of change of the output, we define the dynamics of $\bs_1$ as
\begin{equation}
\label{eq:EDVO_extraDynamics}
J_{\bs_1} \dot{\bs}_1 = \breve{\delta}_{\dot{\by}} \tanh{(\bs_2)},
\end{equation}
where $J_{\bs_1} = \breve{\delta}_{\by} \left( I_n-\tanh^2{\left( \breve{\bs}_1 \right)} \right)$.
According to \eqref{eq:EDVO_outputDefinition} and \eqref{eq:EDVO_extraDynamics}, the time derivative of the output is as
\begin{equation}
\label{eq:BMDVO_outputRateDefinition}
\dot{\by} = J_{\bs_1} \dot{\bs}_1 = \breve{\delta}_{\dot{\by}} \tanh{( \bs_2 )}.
\end{equation}
Thus, if $\bs_2$ is bounded, then $\ |\dot{\by}| < \delta_{\dot{\by}}$.
In conclusion, if the shape state vector of the bounded output programmable oscillator is bounded, we have $\by \in \mathcal{Q}$.

Assuming that ${\bbf(\varphi): \mathbb{R} \rightarrow \mathbb{R}^n}$ is the desired value of $\by$, one can compute the desired value of the shape state vector $\bx = \left[\bs_1^\top,\bs_2^\top\right]^\top$ denoted by $\bx^* (\varphi) = \left[\bg_p^\top (\varphi), \bg_v^\top (\varphi)\right]^\top$ using the inverse of \eqref{eq:EDVO_outputDefinition} and \eqref{eq:BMDVO_outputRateDefinition} as the following
\begin{equation}
\label{eq:BMDVO_stateTransformation}
\begin{aligned}
\mathbf{g}_p (\varphi) &= \tanh^{-1}{\left( \breve{\delta}_{\by}^{-1} \left( \bbf (\varphi) - \by_{avg} \right) \right)}, \\[4pt]
\mathbf{g}_v (\varphi) &= \tanh^{-1}{\left( \breve{\delta}_{\dot{\by}}^{-1} \pbf (\varphi) \right)}.
\end{aligned}
\end{equation}
Consequently, if $\bx$ is bounded and converges to the curve of $\bx^*$ in the shape space, then the output $\by$ converges to the curve of $\bq_d(t) = {\small\left[\bbf^\top(t), \dot{\bbf}^\top(t)\right]^\top}$ in the space $\left(\by,\dot{\by}\right)$ while preserving the output limitations described in \eqref{eq:EDVO_outputConstrained}.
For this purpose, we rewrite the dynamic of the programmable oscillator for the state vector $\left[\bs_1^\top,\bs_2^\top \varphi\right]^\top$ while considering the constraint \eqref{eq:BMDVO_outputRateDefinition} as the following
\begin{subnumcases}{\label{eq:BMDVO_Dynamics}}
J_{\bs_1} \dot{\bs}_1 = \breve{\delta}_{\dot{\by}} \tanh{(s_2)}, \\[5pt]
\begin{aligned}
\dot{\bs}_2 = \, &\bsi_\varphi + \bsi_t - A \be_1 - B \be_2 \\
&- A^{-1}C J_{\bs_1}^{-1} \breve{\delta}_{\dot{\by}} \left( \tanh{(\bs_2)} - \tanh{(\bsi)} \right),
\end{aligned}\\[5pt]
\begin{aligned}
\dot{ \varphi } = 1 + \gamma \Big( \left( \be_1^\top C + \be_2^\top A \right) J_{\bg_p}^{-1} \breve{\delta}_{\dot{\by}} \tanh{(\bg_v)}\\
+ \left( \be_1^\top A + \be_2^\top B \right) \bsi_\varphi \Big), 
\end{aligned} \label{eq:BMDVO_phaseDynamic}\\
\by = \by_{avg} + \breve{\delta}_{\by} \tanh{(\bs_1)},
\end{subnumcases}
where
\begin{align}
&\be_1 = \bs_1 - \mathbf{g}_p, \\
&\be_2 = \bs_2 - \bsi, \\
&\bsi = \tanh^{-1} \left( J_{\bs_1} J_{\bg_p}^{-1} \tanh{(\bg_v)} \right).\label{eq:BMDVO_psiDefinition}
\end{align}
$J_{\bg_p} = \breve{\delta}_{\by} \left( I_n - \tanh^2{\left( \breve{\bg}_p \right)} \right)$, and $A, B, C \in \mathbb{R}^{n\times n}$ and $\gamma \in \mathbb{R}$ are constant coefficients.
$\bsi_\varphi$ and $\bsi_t$ are the partial derivatives of $\bsi$ w.r.t. $t$ and $\varphi$ respectively, and are computed as
\begin{equation}
{\footnotesize
\begin{aligned}
&\bsi_\varphi = J_{\bsi}^{-1} J_{\bs_1} J_{\bg_p}^{-1} \left( 2 \breve{\delta}_{\dot{\by}}^2 J_{\bg_p}^{-1}\tanh^2{(\breve{\bg}_v)} \tanh{(\bg_p)} + J_{\bg_v} \bg_a\right), \\
&\bsi_t = -2 J_{\bsi}^{-1} \breve{\delta}_{\dot{\by}}^2 \tanh{(\breve{\bs}_1)} \tanh{(\bs_2)},
\end{aligned}}
\end{equation}
where
$J_{\bsi} = \breve{\delta}_{\dot{\by}} \left( I_n - \tanh^2{( \breve{\bsi})} \right)$, ${J_{\bg_v} = \breve{\delta}_{\dot{\by}} \left( I_n - \tanh^2{\left( \breve{\bg}_v \right)} \right)}$
and
\begin{equation}
\label{eq:BMDVO_gaDef}
\bg_a = \bg_v^\prime = J_{\bg_v}^{-1} \ppbf (\varphi).
\end{equation}
In the following theorem and remarks, we describe the conditions ensuring the existence of $\bsi$, $J_{\bs_1}$, $J_{\bg_p}$, $J_{\bg_v}$ and $J_{\bsi}$.
\begin{thm}
\label{thm:psiDefinable}
	If $\bbf(t)$ satisfies
	\begin{equation}
	\label{eq:BMDVO_constrainedForPsi}
	{\small
	\breve{\delta}_{\by}^2 \left| \pbf (\varphi) \right| \leq \left| \breve{\delta}_{\by}^2 - \left( \breve{\bbf} (\varphi) - \breve{\by}_{avg} \right)^2\right| \delta_{\dot{\by}}, \quad \forall \varphi \in \left[0,T\right],} %\left| J_{\bg_p}^{-1} \tanh{\left( \bg_v \right)}\right| \le \mathbb{1}_n,
	\end{equation}
	where $T \in \mathbb{R}^+$ is the period of $\bbf(t)$, then the variable $\bsi$ described in \eqref{eq:BMDVO_psiDefinition}, is well-defined.
\end{thm}

The proof is given in Appendix \ref{app:psiDefinable}.

\begin{rmk}
	$J_{\bg_p}$ and $J_{\bg_v}$ are diagonal positive semi definite (PSD) matrices.
	If $\bbf(t) \in \mathcal{Q}$, then $J_{\bg_p}$ and $J_{\bg_v}$ are positive definite (PD), and thus invertible.
\end{rmk}

\begin{rmk}
	$J_{\bs_1}$ is a diagonal PSD matrix.
	If $\bs_1$ is bounded, then $J_{\bs_1}$ is PD, and thus invertible.
\end{rmk}

\begin{rmk}
	$J_{\bsi}$ is a diagonal PSD matrix.
	If $\bbf(t)$ satisfies \eqref{eq:BMDVO_constrainedForPsi}, then $J_{\bsi}$ is PD, and thus invertible.
\end{rmk}

We call the dynamical system presented in \eqref{eq:BMDVO_Dynamics}, bounded output programmable oscillator.
The following theorem concludes the properties of such an oscillator.

\begin{thm}
\label{thm:BMDVO}
	For the bounded output programmable oscillator presented in \eqref{eq:BMDVO_Dynamics}, if
	\begin{itemize}
		\item the function $\bbf(t)$ is a periodic $\mathcal{C}^3$-continuous function and satisfies \eqref{eq:BMDVO_constrainedForPsi},
		\item $A$, $B$ and $C$ are PD diagonal constant matrices, where $BA^{-1}C-A$ is also PD, and
		\item the coefficient $\gamma$ is a nonnegative constant,
	\end{itemize}
then the following results hold
\begin{enumerate}
	\item $\bx(t)$ is bounded and converges to $\bx^*(\varphi)$ from any initial condition;
	\item if $\gamma = 0$, $\left[\bx^{* \top}(t+\varphi(0)),t+\varphi(0)\right]^\top$ is globally AS;
	\item if $\gamma \rightarrow \infty$, $\bx^*(t)$ is the globally stable limit cycle, and
	\item the output $\by(t)$ converges to the curve of $\bq_d(t)$ in the space $\left(\by,\dot{ \by }\right)$ while $\by(t) \in \mathcal{Q}$.
\end{enumerate}
\end{thm}

The proof is given in Appendix \ref{app:BMDVO}.
According to the above theorem, the shape state vector is bounded and converges to $\bx^*$ from any initial condition.
Thus, \eqref{eq:BMDVO_phaseDynamic} converges to $\dot{ \varphi } = 1$.
Therefore, the output $\by(t)$ converges to the curve of $\bq_d(t)$ in $\left(\by, \dot{ \by }\right)$ while $\by(t) \in \mathcal{Q}$.
Moreover, if $\gamma = 0$, the output $\by(t)$ converges to $\bbf(t+\varphi(0))$.
We call the case where $\gamma = 0$, the AS mode.
If $\gamma \rightarrow \infty$, then the bounded output programmable oscillator ensures the global limit cycle tracking of $\bq_d(t)$.
We call the case where $\gamma \gg 1$, the AOS mode.


==> sections/BoundedOutputProgrammableOscillatorWithFeedback.tex <==
\section{BOUNDED OUTPUT PROGRAMMABLE OSCILLATOR WITH INPUT}
\label{sec:feedback}

Using the bounded output programmable oscillator, one can generate a multidimensional smooth trajectory and use it as the reference trajectory for the robot controller.
The generated trajectory tracks the desired one while preserving the predefined limitations for the output and its time derivative.
Though, the important characteristic of CPG technique, \ie the capability of adapting the reference trajectory to disturbances and environment changes, becomes possible by the feedback of the robot and environment information to the CPG.
In this section, we incorporate the sensory feedback to the bounded output programmable oscillator as an external signal.
Then, we investigate the stability properties of the bounded output programmable oscillator dealing with an external signal.

Assume that $\bu \in \mathbb{R}^n$ is an external signal including the robot and environment information.
For integrating $\bu$ with the bounded output programmable oscillator, we modify \eqref{eq:BMDVO_Dynamics} as the following
\begin{equation}
\label{eq:iCPGwithFeedback}
\begin{cases}
J_{\bs_1} \dot{\bs}_1 = \breve{\delta}_{\dot{\by}} \tanh{(s_2)}, \\[7pt]
\begin{aligned}
\dot{\bs_2} = &\, \bsi_\varphi + \bsi_t - A \be_1 - B \be_2\\
& - A^{-1}C J_{\bs_1}^{-1} \breve{\delta}_{\dot{\by}} \left( \tanh{(\bs_2)} - \tanh{(\bsi)} \right) + \bu,
\end{aligned}\\[12pt]
\begin{aligned}
\dot{ \varphi } = 1 + \gamma \left( \left( \be_1^\top C + \be_2^\top A \right) J_{\bg_p}^{-1} \breve{\delta}_{\dot{\by}} \tanh{(\bg_v)} \right.\\
\left. + \left( \be_1^\top A + \be_2^\top B \right) \bsi_\varphi \right), 
\end{aligned}\\[12pt]
\by = \by_{avg} + \breve{\delta}_{\by} \tanh{(\bs_1)},
\end{cases}
\end{equation}
For $\bu = \mathbf{0}_n$, the above dynamic is simplified to \eqref{eq:BMDVO_Dynamics}.
Thus, Theorem \ref{thm:BMDVO} represents the properties of the above dynamic in the absence of $\bu$.
For investigating the properties of the above dynamic in the presence of $\bu$, we compute the dynamic of $\be = \left[\bs_1^\top-\bg_p^\top,\bs_2^\top-\bsi^\top\right]^\top$, called error dynamic, as
\begin{equation}
\label{eq:app_iCPGwithFeedback_errorDyn}
{\small
\begin{cases}
\dot{\be}_1 = J_{\bs_1}^{-1} \breve{\delta}_{\dot{\by}} \tanh{(\bs_2)} - J_{\bg_p}^{-1} \breve{\delta}_{\dot{\by}} \tanh{(\bg_v)} \left(1+\gamma z\right),\\[7pt]
\begin{aligned}
\dot{\be}_2 = -&A \be_1 -B\be_2 - \bsi_\varphi \gamma z + \bu \\
&- A^{-1}C J_{\bs_1}^{-1} \breve{\delta}_{\dot{\by}} \left( \tanh{(\bs_2)} - \tanh{(\bsi)} \right),
\end{aligned}
\end{cases}}
\end{equation}
where
\begin{equation}
\begin{aligned}
z = \left( \be_1^\top C + \be_2^\top A \right) J_{\bg_p}^{-1} \breve{\delta}_{\dot{\by}} \tanh{(\bg_v)} \\
+ \left( \be_1^\top A + \be_2^\top B \right) \bsi_\varphi.
\end{aligned}
\end{equation}
The following theorem explains the properties of the bounded output programmable oscillator in the presence of $\bu$.

\begin{thm}
\label{thm:BMDVO_feedback}
	For the bounded output programmable oscillator presented in \eqref{eq:iCPGwithFeedback} if
	\begin{itemize}
		\item the function $\bbf(t)$ is a periodic $\mathcal{C}^3$-continuous function and satisfies \eqref{eq:BMDVO_constrainedForPsi},
		\item $A$, $B$ and $C$ are positive definite diagonal constant matrices,
		\item $BA^{-1}C-A$ is positive definite, and
		\item the coefficient $\gamma$ is a nonnegative constant,
	\end{itemize}
	then
	\begin{enumerate}
		\item the error dynamic is integral input to state stable (IISS), \ie there exist a $\rho_1 \in \mathcal{KL}$ and a $\rho_2 \in \mathcal{K}_\infty$ such that
		\begin{equation}
		\left\| \be(t) \right\| \leq \rho_2 ( \left\| \be(0) \right\|,t ) + \int_{0}^{t} \rho_2 ( \left\| \bu(s) \right\|) ds.
		\end{equation}
		\item if $\int_{0}^{\infty} \rho_2 \left( \left\| \bu(s) \right\| \right) ds < \infty$, then $\lim\limits_{t \rightarrow \infty} \be(t) = 0$ for any initial condition.
		\item the output preserves the limitations presented in \eqref{eq:EDVO_outputConstrained}, \ie $\by(t) \in \mathcal{Q}$.
	\end{enumerate}
\end{thm}

The proof is given in Appendix \ref{app:BMDVO_feedback}.
The above theorem expresses that if $\int_{0}^{\infty} \rho_2 \left( \left\| \bu(s) \right\| \right) ds < \infty$, then the error signal $\be$ is bounded and converges to $\mathbf{0}_{2n}$ for any initial condition.
Thus, for $\bbf(t) \in \mathcal{Q}$, the shape state vector $\bx$ is bounded and converges to $\bx^*$, and hence the output $\by$ converges to the curve of $\bbf(t)$ in $\left(\by,\dot{\by} \right)$ and is feasible.

==> sections/IntegratedCentralPatternGenerator0.tex <==
\section{Integrated Central Pattern Generator}
\label{sec:integratedCPG}

\begin{figure*}[!t]
	\centering
	\includegraphics[width = 0.98\textwidth]{figures/integratedCPG.jpg}
	\caption{The proposed integrated CPG consisting of a bounded output programmable oscillator with input for generating the reference trajectory of an $n$ dimensional robotic system.}
	\label{fig:integratedCPG}
\end{figure*}

In this section, we introduce the integrated CPG consisting of one bounded output programmable oscillator.
The integrated CPG generates an $n$ dimensional signal $\by$ tracking the $n$ dimensional desired signal $\bbf(t)$ while preserving the predefined limits for $\by$ and $\dot{ \by }$.

The control architecture for a multi degree of freedom robotic system where the reference joint trajectory is generated online using the integrated CPG is depicted in \figurename{\ref{fig:integratedCPG}}.
As can be seen, the high level controller designs the desired motion of the robot, then the motion library determines the desired joint trajectory (\ie $\bq_d(t)$) resulting in the desired motion.
The motion library is a set of the desired joint trajectories having being designed offline for the set of the desired motions supposed to be performed by the robot.
The desired trajectory is used for creating the structure of the integrated CPG.
Using~\eqref{eq:BMDVO_stateTransformation}, the desired limit cycle of the integrated CPG (\ie $(\bg_p(t),\bg_v(t))$) is computed according to the desired trajectory.
After that, the reference joint trajectory is generated by integrating the differential equation of the bounded output programmable that is given in~\eqref{eq:BMDVO_Dynamics}.
The initial condition of the shape states vector of the bounded output programmable oscillator is determined based on the initial condition of the robot by using \eqref{eq:EDVO_outputDefinition} and \eqref{eq:BMDVO_outputRateDefinition}.
The initial condition of the phase state is arbitrary.

According to Theorem \ref{thm:BMDVO}, the integrated CPG generates the desired trajectories satisfying \eqref{eq:BMDVO_constrainedForPsi}.
Considering $\bq_d : \mathbb{R} \rightarrow \mathbb{R}^{2n}$ as the desired trajectory, the schematic of the acceptable region for ${\small\left[\bbf_i,\dot{\bbf}_i\right]}$ where \eqref{eq:BMDVO_constrainedForPsi} is satisfied is depicted in \figurename{\ref{fig:BMDVO_acceptableDesiredFunction}}.
As shown, the acceptable region for ${\small\left[\bbf_i,\dot{\bbf}_i\right]}$ is less than the feasible region for ${\small\left[\by_i,\dot{\by}_i\right]}$ presented in \eqref{eq:EDVO_outputConstrained}.
Thus, the set of acceptable desired trajectories is less than the set of feasible ones ensuring the output limitations.
For generating any feasible desired trajectory, we modify the definition of $\bsi$ as the following
\begin{equation}
\bsi = \tanh^{-1} \left( \hat{\sat} \left( J_{\bs_1} J_{\bg_p}^{-1} \tanh{(\bg_v)} , p \right) \right),
\label{eq:BMDVO_psiDefinitionModify2}
\end{equation}
where $\hat{\sat}(x,p)$ is the continuous estimation of the saturation function $\sat(x)$ and is defined as
\begin{equation}
\hat{\sat}(x,p) = \dfrac{x}{\sqrt[p]{1+|x|^p}}.
\end{equation}
$p \in \mathbb{R}^+$ is a constant.
The behavior of $\hat{\sat}(x,p)$ for different values of $p$ in comparison with $\sat(x)$ is depicted in Fig. \ref{fig:BMDVO_saturationEstimation}.
As can be seen, we have $\lim\limits_{p \rightarrow \infty} \hat{\sat}(x,p) = \sat(x)$.

\begin{figure}[!b]
	\centering
	\includegraphics[width=5.2cm]{figures/BMDVO_acceptableDesiredFunction.jpg}
	\caption{Schematic of the acceptable region for $\bbf_i$ where \eqref{eq:BMDVO_constrainedForPsi} is satisfied. The red dashed lines denote the limitations for $\by_i$ and $\dot{\by}_i$.
		The gray region depicts the acceptable region.}
	\label{fig:BMDVO_acceptableDesiredFunction}
\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=6.3cm]{figures/BMDVO_saturationEstimation.eps}
	\caption{The behavior of $\hat{\sat}(x,p)$ for different values of $p$ w.r.t. $\sat(x)$.}
	\label{fig:BMDVO_saturationEstimation}
\end{figure}
